ACP: An End-to-End Transport Protocol for Delivering Fresh Updates in the Internet-of-Things

The next generation of networks must support billions of connected devices in the Internet-of-Things (IoT). To support IoT applications, sources sense and send their measurement updates over the Internet to a monitor (control station) for real-time monitoring and actuation. Ideally, these updates would be delivered at a high rate, only constrained by the sensing rate supported by the sources. However, given network constraints, such a rate may lead to delays in delivery of updates at the monitor that make the freshest update at the monitor unacceptably old for the application. We propose a novel transport layer protocol, namely the Age Control Protocol (ACP), that enables timely delivery of such updates to monitors, in a network-transparent manner. ACP allows the source to adapt its rate of updates to dynamic network conditions such that the average age of the sensed information at the monitor is minimized. We detail the protocol and the proposed control algorithm. We demonstrate its efficacy using extensive simulations and real-world experiments, which have a source send its updates over the Internet to a monitor on another continent.

==> arch.tex <==
\section{Architecture}

==> cameraReady_texfiles/abstract.tex <==
\begin{abstract}
Internet-of-Things (IoT) applications have sources sense and send their measurement updates over the Internet to a monitor (control station) for real-time monitoring and actuation. Ideally, these updates would be delivered fresh, at a high rate constrained only by the supported sensing rate. However, such a rate may lead to network congestion related delays in delivery of updates at the monitor that make the freshest update at the monitor unacceptably old for the application. Alternately, at low rates, while updates arrive at the monitor with smaller delays, new updates arrive infrequently. Thus, both low and high rates may lead to an undesirably aged freshest update at the monitor.

We propose a novel transport layer protocol, namely the Age Control Protocol (ACP), which enables timely delivery of such updates to monitors over the Internet in a network-transparent manner. ACP adapts the rate of updates from a source such that the average age of updates at the monitor is minimized. We detail the protocol and the proposed control algorithm. We demonstrate its efficacy using extensive simulations and real-world experiments, including wireless access for the sources and an end-to-end connection with multiple hops to the monitor.% To exemplify, ACP achieves about 100 msec of reduction in age in comparison to a baseline that has sources send one update every round-trip-time (RTT). This over a real end-to-end intercontinental connection with round-trip-times of 185 msec.

%This for multiple sources that send their updates over the Internet to monitors on another continent over an end-to-end link with round-trip-times of 185 msec.

%Ideally, a server would desire that the information be delivered at a high rate, only constrained by the rate at which the information can be sensed by the devices. However, given network constraints, such a rate may lead to unacceptable delays at the server. They must be received at a certain rate at the server.Unlike in file transfer or video/voice applications, such monitoring often doesn't require the server to obtain all packets or certain specific packets to be delivered.An application indifferent metric that captures the requirement The server cares to have a good representation of the underlying process. While application specific metrics may be devised... While the  
%The server cares to obtain as fresh as possible a measurement. We propose the Age Control Protocol (ACP), which is a novel transport layer protocol that enables such applications to deliver its updates over the Internet in a transparent manner. Unlike in file transfer or video/voice applications, the server doesn't care for all packets or certain specific packets to be delivered. Instead, it cares for...

%The measurements encapsulate the underlying process of interest. 

%such that they are obtained in a timely manner. for such status updating applications.

%In status updates over internet such as in IoT applications, health sensors, location sensors the freshness of information/update is important rather than the frequency of updates. The updates should be as timely as possible. Sending updates at an arbitrary transmission rate leads to congestion in the network because of the update packets. This leads to increase in age at the receiver. The idea is to avoid congestion while still having fairly recent status updates. In this paper, we propose a congestion control algorithm for the age packets. We propose an Age Control Protocol (ACP) which acts as an orchestration layer between the application and the socket and dictates the rate at which the status updates should be generated so as the minimize the age of the updates at the receiver.

\end{abstract}

==> cameraReady_texfiles/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
%The availability of inexpensive embedded devices with the ability to sense and communicate 
Inexpensive IoT devices have led to the proliferation of a relatively new class of real-time monitoring systems for applications such as health care, smart homes, transportation, and natural environment monitoring. Devices repeatedly sense various physical attributes of a region of interest, for example, traffic flow at an intersection. This results in a device (the \emph{source}) generating a sequence of packets (\emph{updates}) containing measurements of the attributes. A more recently generated update contains a more current measurement. The updates are communicated over the Internet to a \emph{monitor} that processes them and decides on any actuation that may be required. %We assume throughout in this work that the source can generate updates at the desired rate and is not constrained  

For such applications, it is desirable that freshly sensed information is available at monitors. However, simply generating and sending updates at a high rate over the Internet is detrimental to this goal. In fact, freshness at a monitor is optimized by the source smartly choosing an update rate, as a function of the end-to-end network conditions. Freshness at the monitor suffers when a too small or a too large rate of updates is chosen by the source. See, for example,~\cite[Figure 3]{KaulYatesGruteser-Infocom2012} for how age at the monitor varies as a function of source rate for simple first-come-first-served queues with memoryless arrival and service processes.

%Figure~\ref{fig:networkingMetrics} broadly captures the behavior of the metrics of delay and age as a function of throughput. Under light and moderate loads when packet dropping is negligible, throughput (average network utilization) increases linearly in the rate of updates. This leads to an increase in the average packet delay. Large packet delays coincide with large average age. Large age is also seen for small throughputs (and corresponding small rate of updates). \emph{At a low update rate, the monitor receives updates infrequently, and this increases the average age (staleness) of its most fresh update}. Finally, observe that there exists a sending rate (and corresponding throughput) at which age is minimized.

%We propose the Age Control Protocol (ACP), which in a network-transparent manner regulates the rate at which updates from a  source are sent over its end-to-end connection to the monitor. This rate is such that the average age, where the age of an update is the time elapsed since its generation by the source, of sensed information at the monitor is kept to a minimum, given the network conditions. Based on feedback from the monitor, ACP adapts rate to the perceived congestion in the Internet. Consequently, ACP also limits congestion that would otherwise be introduced by sources sending to their monitors at unnecessarily fast update rates. %(SKK: Something about the network not being known?)
%\begin{figure}[!t]             
%\begin{center}
%\includegraphics[width=0.3\textwidth]{Figs/currentIoT5.pdf}
%\caption{\textcolor{green}{Unlike the traditional applications like voice, video or file download; real-time monitoring applications are highly loss resilient and care for freshness of an update. Existing transport protocols like TCP and RTP are not best suited for such applications.}}
%\label{fig:currentIoT}
%\end{center}
%\end{figure}
%Figure~\ref{fig:monitoringApp} illustrates such monitoring applications coexisting with other applications like voice, video, and file transfers, which all share the Internet. %This also determines the network bandwidth used and the obtained voice/video quality.

The requirement of freshness is not akin to requirements of other pervasive real-time applications like voice and video. While resilient to packet drops to a certain degree, they require end-to-end packet delays to lie within known limits and would like small end-to-end jitter. Monitoring applications may achieve a low update packet delay by simply choosing a low rate at which the source sends updates. This, however, may be detrimental to freshness, as a low rate of updates can lead to a large \emph{age} of sensed information at the monitor, simply because updates from the source are infrequent. More so than voice/video, monitoring applications are exceptionally loss resilient and they don't benefit from the source retransmitting lost updates. Instead, the source should continue sending new updates at its configured rate.
%\begin{figure}[!t]             
%\begin{center}
%\includegraphics[width=0.4\textwidth]{Figs/ageThrDelay.pdf}
%\caption{Interplay of the networking metrics of delay (solid line), throughput (normalized by service rate) and age. Shown for a M/M/1 queue~\cite{shortle2018fundamentals} with service rate of $1$. The age curve was generated using the analysis for a M/M/1 queue in~\cite{KaulYatesGruteser-Infocom2012}.}
%\label{fig:networkingMetrics}
%\end{center}
%\vspace{-0.2in}
%\end{figure}

At the other end of the spectrum are applications like that of file transfer that require reliable transport and high throughputs but are delay tolerant and use the transmission control protocol (TCP). The congestion control algorithm of TCP, which optimizes the use of the network pipe for throughput, is detrimental to keeping age low. We detail the impact of TCP on age in \cite[Section 3]{shreedhar_wowmom_long}\footnote{We don't include evaluation of TCP in this paper because of limited space.}. Its features of packet retransmissions and in-order delivery can keep fresh packets waiting at the monitor TCP for older packets to be successfully received. This causes large increases in age on transmission errors. Also, small sized updates may age more than larger ones as the congestion window size doesn't increase till a sender maximum segment size bytes are acknowledged. This delays the delivery of updates with fewer bytes.% require multiple TCP ACK(s) to be received for the congestion window to increase. This delays their delivery to the monitor. 

Unlike TCP, UDP ignores dropped packets and delivers packets to applications as soon as they are received. This makes it desirable for age sensitive applications. In fact, while ACP chooses the best rate of sending updates, it uses UDP to transport them over the Internet.
%Specifically, we have evaluated the impact of (a) TCP features of packet retransmissions and in-order delivery and (b) its handling of small packets by the TCP congestion control. 

Our specific contributions are listed next.
%TCP via its congestion control mechanism attempts to keep as many application bytes in transit over the end-to-end connection as is possible without packet drops due to network congestion. For updating applications, TCP is detrimental to optimizing freshness as it tries by design to fill the network pipe. This increases throughput but also increases packet delay because of queueing. Such a strategy would correspond to the source sending updates at a high rate. While the monitor would receive a steady stream of updates at the high rate, each update would have a high age, when received by the monitor, as a result of it having experienced a large network delay.


%While the server may receive a steady rate of updates (a large throughput), the updates will be delayed as a result of the congestion. %These applications are distinct from that of file transfer and real-time voice/video. Such an application would desire that the monitor has the most currently sensed update at any given time. However, the same may not be feasible given constraints imposed by the communications network. To elucidate, let's say the source sends fresh updates at a rapid rate. However, the faster the rate of updates, the larger the throughput, and the larger is the average delay (Figure~\ref{fig:networkingMetrics}) with which an update is received at the monitor. This is explained by the larger resulting congestion in the network. As a result, the freshest update at the monitor at any given time will be stale, that is of large age.

%Figure~\ref{fig:networkingMetrics} broadly captures the behavior of the metrics of delay and age as a function of throughput. Under light and moderate loads when packet dropping is negligible, throughput (average network utilization) increases linearly in the rate of updates. This leads to an increase in the average packet delay. Large packet delays coincide with large average age. Large age is also seen for small throughputs (and corresponding small rate of updates). \emph{At a low update rate, the monitor receives updates infrequently, and this increases the average age (staleness) of its most fresh update}. Finally, observe that there exists a sending rate (and corresponding throughput) at which age is minimized.
%SKK [checking for space]
%\begin{figure*}[!th]
%	\begin{center}
%		\subfloat[]{\includegraphics[width=.33\textwidth]{MATLAB_plots_WoWMoM/Fig1a_ageUDP_TCP_retrans_skk.eps}
%			\label{fig:UDPvsTCPPacketError}}
%		%\hspace{-0.1in}
%		\subfloat[]{\includegraphics[width=.33\textwidth]{MATLAB_plots_WoWMoM/rxBytes_delay_skk.eps}
%			\label{fig:UDPvsTCPPacketErrorRXBuffer}}
%		\subfloat[]{\includegraphics[width=.33\textwidth]{MATLAB_plots_WoWMoM/Fig1c_tcp_500_536B_skk.eps}
%			\label{fig:TCPSmallPacketSizes}}
%		\label{fig:TCPEval}
%		\caption{(a) Impact of packet errors on age and packet delay when using TCP and UDP (b) A time snapshot of delays suffered by update packets transmitted using TCP and the corresponding received bytes by the monitor. Packet error rate was set to $0.1$ (c) Age as a function of packet size and how packet size impacts increase of the TCP congestion window.}
%	\end{center}
%	\vspace{-0.2in}
%\end{figure*}

\noindent \textbf{(a)} We propose the Age Control Protocol (detailed in Sections~\ref{sec:ACPProtocol},~\ref{sec:problem},~\ref{sec:acpIntuit}, and~\ref{sec:algorithm}), a novel transport layer protocol for real-time monitoring applications that aims to deliver fresh updates over the Internet. ACP regulates the rate at which a source sends its updates to a monitor over its end-to-end connection in a manner that is application independent and makes the network transparent to the source. 

The goal is to keep the average age of sensed information at the monitor to a minimum, where the age of an update is the time elapsed since its generation by the source. Based on feedback from the monitor, ACP adapts rate to the perceived congestion in the Internet. Consequently, ACP also limits congestion that would otherwise be introduced by sources sending to their monitors at unnecessarily fast update rates. We argue that ACP, unlike other transport protocols like TCP and RTP, must maintain just the right number of update packets in transit at any given time.

%\noindent \textbf{(b)} We demonstrate in Section~\ref{sec:TCP} that TCP, which is the most commonly used transport protocol in the Internet is not suitable for the transport of updates for real-time monitoring. 

\noindent \textbf{(b)} We provide an extensive evaluation of ACP (Sections~\ref{sec:evaluation},~\ref{sec:simulationResults} and ~\ref{sec:realWorldResults}) using network simulations and real-world experiments in which one or more sources sends packets to monitors. To exemplify, over an inter-continental end-to-end IP connection with a median round-trip-time of about $185$ msec, ACP achieves a significant reduction in the median age of about $100$ msec ($\approx 33\%$ improvement) over age achieved by a protocol that sends one update every RTT.


We end this section with a brief on the related art. Prior works~\cite{KaulYatesGruteser-Infocom2012,KamKompellaEphremides2013ISIT,KamKNE2016IT} have analyzed the metric of age of sensed information (AoI) for queue theoretic abstractions of networks. Works have considered optimizing age for multiple sources sharing a communication link, for example, \cite{Kadota-UBSM-Allerton2016,JiangKrishnmachariZZN-ISIT2018}. AoI has been analyzed under a variety of link scheduling methods \cite{LuJiLi-Mobicom2018,Talak-KKM-arxiv2018}. Multihop networks have also received attention \cite{TalakKaramanModiano-Allerton2017}. Notably, optimality properties of a Last Generated First  Served service when updates arrive out of order are found in \cite{Bedewy-SS-arxiv2017}. 

Such AoI literature has focused on analytically tractable simple models. Moreover, a model for the system is typically assumed to be known. In this work, our objective has been to develop end-to-end updating schemes that perform reasonably well without assuming a particular network configuration or model. Closer to our goal, more recently, in~\cite{sert2018DeepQ} the authors proposed a deep Q-learning based approach to optimize age over a given but unknown network topology. A preliminary version of our work on ACP appeared as a poster~\cite{shreedhar2018acp}.
%\noindent \textbf{(d)} We show that ACP adapts the source update rate to make effective use of a fast end-to-end path with multiple hops from the source to the monitor. Over a connection with a median round-trip-time of about $185$ msec, ACP achieves a significant reduction in median age of about $100$ msec ($\approx 33\%$ improvement) over age achieved by a protocol that sends one update every round-trip-time.
%\end{enumerate}
%The rest of the paper is organized as follows. In the next section, we describe related works. In Section~\ref{sec:TCP} we demonstrate why the mechanisms of TCP are detrimental to minimizing age. In Section~\ref{sec:ACPProtocol}, we detail the Age Control Protocol, how it interfaces with a source and a monitor, and the protocol's timeline. In Section~\ref{sec:problem} we define the age control problem. In Section~\ref{sec:acpIntuit}, we use simple queueing models to intuit a good age control protocol and discuss a few challenges. Section~\ref{sec:algorithm} details the control algorithm that is a part of ACP. This is followed by details on the evaluation methodology in Section~\ref{sec:evaluation}. We discuss simulation results in Section~\ref{sec:simulationResults} and results from real-world experiments in Section~\ref{sec:realWorldResults}. We conclude in Section~\ref{sec:conclusions}.

%%\begin{figure*}[!t]
%%\begin{center}
%%\subfloat[]{\includegraphics[width=0.42\textwidth]{Figs/NetworkStack}\label{fig:networkStack}}
%%\hspace{0.1in}
%%\subfloat[]{\includegraphics[width=0.48\textwidth]{Figs/age.pdf}\label{fig:ageSampleFunction}}
%%\caption{(a) The ACP end-to-end connection. (b) A sample function of the age process $\age(t)$. Updates are indexed $1,2,\ldots,n$. When representative of the age process at the monitor, $a_i$ is the time at which update $i$ was sent by the source and $d_i$ is the time the update was received at the corresponding monitor. In case, the age process at the monitor is being estimate by the source ACP, $d_i$ is the time the ACK for update $i$ was received by the ACP.}
%%\label{fig:networkStackAndAgeSample}
%%\end{center}
%%\end{figure*}



%ACP suggests to a source the rate at which it must send fresh updates such that the average age at the monitor is minimized. ACP adapts its suggestion to the perceived congestion in the Internet. By suggesting this desired rate to a source, ACP also limits congestion that may be introduced by an unnecessarily fast rate of updates sent by sources to their monitors.

%Updates that are lost due to network congestion or link errors don't affect the age at the server.
%%ACP: congestion dynamic adaptation and avoidance.... congests the network appropriately.. keeps unnecessary updates to a minimum.
%%
%%We envision ACP to play a role of the kind RTP has played for real-time applications. Such applications need ACP.
%%
%%While extensive knowledge of the process being sensed and the network may help devise better metrics...
%Works on age... Application specific interventions (Yin's work)... Dynamic prog approach...
%Also~\cite{van_red}

%%Age sawtooth figure.. resets need to explained... out-of-order delivery ... errors .... the $\age(t)$ definition must be provided.
%%Age, delay, and throughput for M/M/1.... Say how age changes with update rate....
%%Age as a metric... why it is good... % Yin's work as an application specific...
%%The general optimization problem... maybe linked to the definition of $\age(t)$ as a stochastic process
%%RTP, TCP
%%Since not every packet is important... ACP used UDP
%%RTP~\cite{schulzrinne2003rtp} caters to real-time applications like voice and video and allows them to provide source coding information and in addition provides QoS information that can help the applications adapt their encoding to the network.
%%%In this section we will discuss the following
%%%IoT applications, 
%%%importance of age as a metric,
%%%difference between throughput and age as a metric,
%%%and hence motivation age,
%%%sawtooth pattern of age curve 
%%%congestion control
%%%
%%%The contributions of this paper are:
%%%
%%%\begin{enumerate}[(a)]
%%%\item We propose Age Control Protocol, which a novel congestion control protocol for age packets. It solves the problem of congestion in the network due to arbitrary transmission rate of the status updates while still having fairly recent status updates.
%%%
%%%\item We provide ACP as an orchestration layer between the application and the socket which dictates the rate at which the status updates should be generated so as to minimize the age of the status update at the receiver.
%%%
%%%\item We motivate the need of ACP using a client server sending status updates at different rates. We see that the age is minimized at a specific rate and increases on increasing or decreasing the rate.
%%%
%%%\item We test our algorithm in both simulation as well as in real set-up.
%%% 
%%%\end{enumerate}
%Rest of the paper is organized as follows. We discuss the relevant background and related works in Section~\ref{sec:relatedwork}. Section - motivates the need for age control protocol. 
%In applications such as remote sensing, environmental sensing etc status updates are sent to interested recipients. Ideally these update should be received as timely as possible. Intuitively, sending updates as soon as possible might seem like a good policy. However it, as discussed in detail later in the paper, might lead to self congestion in the network due to the age packets in the system. In this paper, we propose a Age Control Protocol based on the age metric.

==> cameraReady_texfiles/intuition.tex <==
\section{Good Age Control Behavior and Challenges}
\label{sec:acpIntuit}
%%\begin{figure}[thb]             
%%	\begin{center}
%%		\subfloat[]{\includegraphics[width=.23\textwidth]{MATLAB_plots_WoWMoM/UDP_baselines_AllTopology.eps}
%%		\label{fig:motivatingACP_age_lambda}}
%%		\subfloat[]{\includegraphics[width=.23\textwidth]{Figs/BacklogAndQueues.pdf}
%%		\label{fig:motivatingACPBacklog}}
%%	\end{center}
%%\end{figure}
%\begin{figure}[thb]             
%	\begin{center}
%			\includegraphics[width=.5\textwidth]{MATLAB_plots_WoWMoM/optimal_backlog_skk.eps}
%			\caption{Average backlogs at different nodes in the network, shown in Fig~\ref{fig:simulationNetwork}, at the optimal update rate. Net E is similar to Net A and not shown.}
%			\label{fig:motivatingACPBacklog}
%	\end{center}
%\vspace{-0.1in}
%\end{figure}
%%\begin{figure}[thb]
%%	\begin{center}
%%		\includegraphics[width=.32\textwidth]{Figs/BacklogAndQueues.pdf}
%%		\caption{??}
%%		\label{fig:motivatingACPBacklog}
%%	\end{center}
%%\end{figure}
%
%\begin{table}
%	\begin{center}
%		\begin{tabular}[thb]{|L|L|L|L|L|L|L|}
%			\hline
%			\text{Network} & R_1 & R_2 & R_3 & R_4 & R_5 & R_6\\
%			%	\hline
%			%	\text{Net A} & 1 & 1 & 1 & 1 & 1 & 1 & 0\\
%			\hline
%			\text{Net A} & 1 & 1 & 1 & 1 & 1 & 1\\
%			\hline
%			\text{Net B} & 1 & 1 & \mathbf{5} & \mathbf{5} & 1 & 1\\
%			\hline
%			\text{Net C} & 1 & \mathbf{5} & 5 & 5 & \mathbf{5} & 1\\
%			\hline
%			\text{Net D} & \mathbf{5} & 5 & 5 & 5 & 5 & 1\\
%			\hline	
%			\text{Net E} & 5 & 5 & 5 & 5 & 5 & \mathbf{5}\\
%			\hline
%		\end{tabular}
%		\caption{Various P2P link configurations applied to the network diagram in Figure~\ref{fig:simulationNetwork}. The rates $R_i$ are in Mbps. $R_1$ is the rate of the link between the source and AP-1 and $R_6$ is that of the link between AP-2 and the monitor.}
%		\label{tab:goodACPSimulationTable}
%	\end{center}
%\vspace{-0.2in}
%\end{table}
%%\begin{figure}[ht]             
%%	\begin{center}
%%		\includegraphics[width=.32\textwidth]{MATLAB_plots_WoWMoM/UDP_baselines_AllTopology.eps}
%%		\caption{??}
%%		\label{fig:motivatingACP_age_lambda}		
%%	\end{center}
%%\end{figure}
ACP must suggest a rate $\lambda$ updates/second at which a source must send fresh updates to its monitor. ACP must adapt this rate to network conditions. To build intuition, let's suppose that the end-to-end connection is well described by an idealized setting that consists of a single first-come-first-served (FCFS) queue that serves each update in constant time.  An update generated by the source enters the queue, waits for previously queued updates, and then enters service. The monitor receives an update once it completes service. Note that every update must age at least by the (constant) time it spends in service before it is received by the monitor. It may age more if it ends up waiting for one or more updates to complete service. 

In this idealized setting, one would want a new update to arrive as soon as the last generated update finishes service. To ensure that the age of each update received at the monitor is the minimum, one must choose a rate $\lambda$ such that new updates are generated in a periodic manner with the period set to the time an update spends in service. Also, update generation must be synchronized with service completion instants so that a new update enters the queue as soon as the last update finishes service. In fact, such a rate $\lambda$ is age minimizing even when updates pass through a sequence of $Q>1$ such queues in tandem~\cite{shortle2018fundamentals}. The update is received by the monitor when it leaves the last queue in the sequence. The rate $\lambda$ will ensure that a generated packet ages exactly $Q$ times the time it spends in the server of any given queue. At any given time, there will be exactly $Q$ update packets in the network, one in each server.% An illustration shown in Figure~\ref{fig:goodACP}. 

Of course, the assumed network is a gross idealization. We assumed a series of similar constant service facilities and that the time spent in service and instant of service completion were known exactly. We also assumed lack of other traffic. However, the resulting intuition is significant. Specifically, \emph{a good age control algorithm must strive to have as many update packets of a source in transit as  possible while simultaneously ensuring that these updates avoid waiting for other previously queued  updates of the source}\footnote{Simulations that further build on this intuition may be found in~\cite{shreedhar_wowmom_long}. We skip them here due to lack of space.}.

As described next, ACP tracks changes in the number of backlogged packets, which are updates for whom the source awaits an ACK from the monitor, and average age over short intervals. In case backlog and age increase, ACP acts to rapidly reduce the backlog.

%%To build on this intuition we simulated an end-to-end connection which has the source send its packet to the monitor over $6$ hops, where each hop is serviced by a bidirectional P2P link. The hops are shown in Figure~\ref{fig:simulationNetwork}. We vary the rates at which the P2P links transmit packets to gain insight into how queues in a network must be populated with update packets at an age optimal rate. We also introduce other traffic in the network that occupies, on an average, a fraction $0.2$ Mbps of each P2P link from the source to the monitor. The different configurations are summarized in Table~\ref{tab:goodACPSimulationTable}. For each network configuration we have the source send updates over UDP to the monitor using an a priori chosen rate $\lambda$. We vary $\lambda$ over a wide range of values and for each $\lambda$ we calculate the obtained time average age. These simulations allow us to empirically pick the age minimizing $\lambda$ for the given network. %This average age as a function of $\lambda$ is shown for Net B and Net F in Figure~\ref{fig:motivatingACP_age_lambda}. 

%%Figure~\ref{fig:motivatingACPBacklog} shows the time average \emph{backlog} (queue occupancy) at the different nodes in the network at the optimal $\lambda$. The backlog at a node includes the update packet being transmitted on a node's outgoing P2P link and any update that is awaiting transmission at the node. Observe that all P2P links in each of Net A and Net E have the same rate, $1$ and $5$ Mbps respectively. Though Net B has links much faster than that of Net A, for both these networks the average backlog at all nodes is close to $1$. That it is smaller than $1$ is explained by the presence of the other flow. The other flow, which also originates at the client, is also the reason why the client sees a slightly larger average queue occupancy by the update packets.% Once a packet, update or otherwise, leaves the client it doesn't wait for other packets to finish transmission and is transmitted right away.%  In the absence of the other flow, we have observed (not shown) that the average queue occupancy in queues at all the nodes approaches $1$ as $\lambda$ gets closer to the optimal.

%%Net B has faster P2P links connecting ISP(s) and the Gateway when compared to Net A. However, its other links are slower than that in Net E. We see that the nodes that have fast outgoing links have low backlogs and those that have slow links have an average backlog close to $0.8$. The source has a slow outgoing link and as a result of the other flow sees slightly larger occupancy of update packets. In summary, at $\lambda$ that minimizes average age, as is also shown in Figure~\ref{fig:motivatingACPBacklog} for Net C and Net D, \emph{nodes with outgoing links that are bottlenecks relative to the others' links see a backlog such that no more than one update packet is queued at them}. Naturally, nodes with faster links see smaller backlogs in proportion to how fast their links are with respect to the bottleneck.

%%A corollary to the above observations, which we do not demonstrate for lack of space, is that a good age control algorithm should on an average have a larger number of packets simultaneously in transit in a network with a larger number of hops (nodes/queues).

%We end this section with a discussion of Figure~\ref{fig:motivatingACP_age_lambda}, which shows how average age changes with $\lambda$ for the networks Net A and Net E. Note that the minimum average age obtained in Net E is about $5\times$ smaller than that obtained in Net A. This is explained by smaller end-to-end delays experienced by packets in Net E because of its links that are $5 \times$ faster than the corresponding links in Net A. What is more interesting, however, is the big shift in the $\lambda$ that minimizes the average as we go from slower links (think congested network) to faster links (think lightly loaded network). This further motivates the need for a good age control protocol that quickly adapts to changing network conditions. In fact, at the $\lambda$ that is optimal for Net E, Net A sees very large average age. This is because nodes in Net A see high backlogs of update packets waiting in their queues.  

%A good age control algorithm must not allow the end-to-end connection to drift into a high backlog state. As described next, ACP tracks changes in the number of backlogged packets and average age over short intervals, and in case backlog and age increase, ACP acts to rapidly reduce the backlog.

%We consider the following network configurations: (a) \emph{Net A:} Each P2P link has a rate of $1$ Mbps and the only traffic that occupies the links in the network is from the source. This network is thus similar to the idealization we discussed above. (b) \emph{Net B:} This network differs from \emph{Net A} only in that it has another end-to-end UDP flow that occupies on an average a fraction $0.2$ of each $1$ Mbps P2P link. (c) \emph{Net C:} Like \emph{Net B} other than the P2P links that connect the gateway to ISP1 and ISP2, which have rates of $5$ Mbps instead of $1$ Mbps. (d) \emph{Net D:} The P2P links that connect the source and its AP and the monitor and its AP are $1$ Mbps. All other links are $5$ Mbps. (e) \emph{Net E:}.
%Before we detail our proposed control method, we will make a few salient observations using analytical results for simple queueing models that capture stochastic service and generation of updates. These will help build on our intuition and also elucidate the challenges of age control over a priori unknown and likely non-stationary end-to-end network conditions. 
%
%We will consider two queueing models. One is the $M/M/1$ FCFS queue with an infinite buffer in which a source sends update packets at a rate $\lambda$ to a monitor via a single queue, which services packets at a rate $\mu$ updates per second. The updates are generated as a Poisson process of rate $\lambda$ and packet service times are exponentially distributed with $1/\mu$ as the average time it takes to service a packet. In the other model, updates travel through two queues in tandem. Specifically, they enter the first queue that is serviced at the rate $\mu_1$. On finishing service in the first queue, they enter the second queue that services packets at a rate of $\mu_2$. As before, updates arrive to the first queue as a Poisson process and packet service times are exponentially distributed. The average age for the case of a single $M/M/1$ queue was analyzed in~\cite{KaulYatesGruteser-Infocom2012}. We extend their analysis to obtain analytical expressions of average age as a function of $\lambda,\mu_1$ and $\mu_2$ for the two queue case, by using the well known result that updates also enter the second queue as a Poisson process of rate $\lambda$~\cite{shortle2018fundamentals}.%, from the analysis of series queues~\cite{DonaldGross}.


%\emph{On the impact of non-stationarity and transient network conditions:} 
%Figure~\ref{fig:motivatingACP_age_lambda} shows the expected value (average) of age as a function of $\lambda$ when the queueing systems are in \emph{steady state}. It is shown for three single $M/M/1$ queues, each with a different service rate, and for two queues in tandem with both servers having the same unit service rate. Observe that all the age curves have a bowl-like shape that captures the fact that a too small or a too large $\lambda$ leads to large age. Such behavior has been observed in non-preemptive queueing disciplines in which updates can't preempt other older updates. A reasonable strategy to find the optimal rate thus seems to be one that starts at a certain initial $\lambda$ and changes $\lambda$ in a direction such that a smaller expected age is achieved. 
%
%In practice, the absence of a network model (unknown service distributions and expectations), would require Monte-Carlo estimates of the expected value of age for every choice of $\lambda$. Getting these estimates, however, would require averaging over a large number of instantaneous age samples and would slow down adaptation. This could lead to updates experiencing excessive waiting times when $\lambda$ is too large. Worse, transient network conditions (a run of bad luck) and non-stationarities, for example, because of introduction of other traffic flows, could push these delays to even higher values, leading to an even larger backlog of packets in transit. Figure~\ref{fig:motivatingACP_age_lambda}, illustrates how changes in network conditions (service rate $\mu$ and number of hops (queues)) can lead to large changes in the expected age.
%
%It is desirable for a good age control algorithm to not allow the end-to-end connection to drift into a high backlog state. As we describe in the next section, ACP tracks changes in the average number of backlogged packets and average age over short intervals, and in case backlog and age increase, ACP acts to rapidly reduce the backlog.

%\emph{On Optimal Average Backlogs:} Figure~\ref{fig:motivatingACPArrivalAndSystem} plots the average packet system times, where the system time of a packet is the time that elapses between its arrival and completion of its service, as a function of inter-arrival time ($1/\lambda$) for three single queue $M/M/1$ networks and two networks that have two queues in tandem. As expected, increase in inter-arrival time reduces the system time. As inter-arrival times become large, packets wait less often for others to complete service. As a result, as inter-arrival time increases, the system times converge to the average service time of a packet. For each queueing system, we also mark on its plot the inter-arrival time that minimizes age. It is instructive to note that for the three single queue systems this inter-arrival time is only slightly smaller than the system time. However, for the two queues in tandem with service rates of $1$ each, the inter-arrival time is a lot smaller than the system time. The implication being that on an average it is optimal to send slightly more than one ($\approx 1.2$) packet every system time for the single queue system. However, for the two queue network with the similar servers, we want to send a larger number ($\approx 1.6$) of packets every system time. For the two queue network where the second queue is served by a faster server, this number is smaller ($\approx 1.43$). As we observe next, as one of the servers becomes faster, the two queue network becomes more akin to a single queue network with the slower server.
%
%Note that these numbers are in fact the optimal (age minimizing) average number of packets in the system. Figure~\ref{fig:motivatingACPBacklog} shows how this optimal average backlog varies as a function of $\mu_2$ for a given $\mu_1$. The observations stay the same on swapping $\mu_1$ and $\mu_2$. As $\mu_2$ increases, that is as the second server becomes faster than the first ($\mu_1 = 1$), we see that the average backlog increases in queue $1$ and reduces in queue $2$, while the sum backlog gets closer to the optimal backlog for the single queue case. Specifically, as queue $1$ becomes a larger bottleneck relative to queue $2$, optimal $\lambda$ must adapt to the bottleneck queue. The backlog in the faster queue is governed by the resulting choice of $\lambda$. For when the rates $\mu_1$ and $\mu_2$ are similar, they see similar backlogs. However, as is seen for when $\mu_1,\mu_2 = 1$, the backlog per queue is smaller than a network with only a single such queue. However, the sum backlog ($\approx 1.6$) is larger. 
%To summarize, one would want a good age control algorithm to have a larger number of packets simultaneously in transit in a network with a larger number of hops (queues).



%Independent from service rate. It is about the number you want in a queue.... If service gets faster, increase rate... Keep the backlog at the optimal.
%For the rate that is modulated by the bottleneck link, the average time that a packet spends in the faster service queue is small. This leads to a smaller average occupancy of the faster queue by the updates.
%How many packets must be in transit at any given time?
%ACP tries to achieve the desired level of backlog.... it does so by ensuring that change in backlog is in the correct direction...
%Drift: (a) the example that motivated going from action (1) to (2). (b) Even before this, we saw drift. For example, if depTime changes.... you may not get the desired change in backlog.... A more serious situation is that the direction of change is as wanted... however, the amount is just noise.
%Too large a ctrl interval.... motivated min(RTT, depTime)... show linear increase with backlog... for RTT
%Too small a step size is bad... (A very small step size may not change anything wrt age)...
%\begin{figure*}[!ht]             
%	\begin{center}
%		\subfloat[]{\includegraphics[width=.32\textwidth]{MATLAB_plots_WoWMoM/UDP_baselines_AllTopology.eps}
%			\label{fig:motivatingACP_age_lambda}}
%		\hspace{.001in}
%		\subfloat[]{\includegraphics[width=.32\textwidth]{Figs/ArrivalTime_SystemTime_different_mu-b.pdf}
%			\label{fig:motivatingACPArrivalAndSystem}}
%		\hspace{.001in}
%		\subfloat[$\mu_1 = 1.$]{\includegraphics[width=.32\textwidth]{Figs/BacklogAndQueues.pdf}
%			\label{fig:motivatingACPBacklog}}
%		\caption{(a) Expected value of age as a function of update rate $\lambda$ is shown for different queueing networks. (b) Average update packet system time is shown as a function of inter-arrival time ($1/\lambda$). The green dashed line is the $45^{\circ}$ line. The $\mathrel +$ mark the age minimizing $\lambda$. (c) The backlog in each queue and the sum is shown as the service rate of the second queue increases from $1$ to $5$. Service rate of the first queue is $\mu_1 = 1$.}
%		\label{fig:motivatingACP}
%	\end{center}
%\end{figure*}

==> cameraReady_texfiles/whynotTCP.tex <==
\section{Age Sensitive Update Traffic over TCP}
\label{sec:TCP}
Before we delve into the problem of end-to-end age control, we demonstrate why TCP as a choice of transport protocol is unsuitable for age sensitive traffic. Specifically, we show that the congestion control mechanism of TCP together with its goal of guaranteed and ordered delivery of packets can lead to a very high age at the monitor, in comparison to when UDP is used, for a wide range of utilization of the network by the traffic generated by the source, and not just when the utilization is high.

We simulated a simple network consisting of a source that sends measurement updates to a monitor via a single Internet Protocol (IP) router. The source node has a bidirectional point-to-point (P2P) link of rate $1$ Mbps to the router. A similar link connects the router to the monitor. The source uses a TCP client to connect to a TCP server at the monitor and sends its update packets over the resulting TCP connection. We will also compare the obtained age with when UDP is used instead.

\emph{Retransmissions and In-order Delivery:} Figure~\ref{fig:UDPvsTCPPacketError} illustrates the impact of packet error on TCP. A packet was dropped independently of other packets with probability $0.1$. The figure compares the average age at the monitor and the average update packet delay, which is the time elapsed between generation of a packet at the source and its delivery at the monitor, when using TCP and UDP. On using TCP, the time average age achieves a minimum value of $0.18$ seconds when the source utilizes a fraction $0.2$ of the available $1$ Mbps to send update packets. This is clearly much larger than the minimum age of $\approx 0.01$ seconds at a utilization of $\approx 0.8$ when UDP is used. 

The large minimum age when using TCP is explained by the way TCP guarantees in order packet delivery to the receiving application (monitor). It causes fresher updates that have arrived out-of-order at the TCP receiver to wait for older updates that have not yet been received, for example, because of packet losses in the network. This can be seen in Figure~\ref{fig:UDPvsTCPPacketErrorRXBuffer} that shows how large measured packet delays coincide with a spike in the number of bytes received by the monitor application. The large delay is that of a received packet that had to undergo a TCP retransmission. The corresponding spike in received bytes, which is preceded by a pause, is because bytes with fresher information received earlier but out of order are held by the TCP receiver till the older packet is received post retransmission. Unlike TCP, UDP ignores dropped packets and delivers packets to applications as soon as they are received. This makes it desirable for age sensitive applications. As we will see later, ACP uses UDP to provide update packets with end-to-end transport over IP.

\emph{TCP Congestion Control and Small Packets:} Next, we describe the impact of small packets on the TCP congestion algorithm and its impact on age. This is especially relevant to a source sending measurement updates as the resulting packets may have small application payloads. Note that no packet errors were introduced in simulations used to make the following observations. Observe in the upper plot of Figure~\ref{fig:TCPSmallPacketSizes} that the $500$ byte packet payloads experience higher age at the monitor than the larger $536$ byte packets. The reason is explained by the impact of packet size on how quickly the size of the TCP congestion window (CWND) increases. The congestion window size doesn't increase till a sender maximum segment size (SMSS) bytes are acknowledged. TCP does this to optimize the overheads associated with sending payload. Packets with fewer bytes may thus require multiple TCP ACK(s) to be received for the congestion window to increase. This explains the slower increase in the size of the congestion window for $500$ byte payloads seen in Figure~\ref{fig:TCPSmallPacketSizes}. This causes smaller packets to wait longer in the TCP send buffer before they are sent out by the TCP sender, which explains the larger age in Figure~\ref{fig:TCPSmallPacketSizes}.

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

%The efficiency of MPTCP is largely dependent on effectiveness of the path scheduler.  In this paper, we argue that a scheduler's reliance on only TCP-level information doesn't fully exploit the available network capacity and a more holistic approach to MPTCP is needed. 

%The performance of MPTCP is largely dependent on effectiveness of its scheduler.  

%We proposed a novel MPTCP scheduler, QAware, which adopts a cross-layer approach to the scheduling problem. We showed that relying on only TCP-level information to make scheduling decisions doesn't fully utilize the aggregate network bandwidth available to an application over multiple network interfaces. 

We proposed, QAware, a novel cross-layer MPTCP scheduler that combines hardware device queue occupancy and TCP RTT for efficient scheduling decisions. We detailed its design and implementation. We evaluated QAware using an extensive set of simulations and real network experiments for various network configurations and applications such as bulk data transfers, web browsing, web file downloads, and video streaming. Comparisons with various state-of-the-art schedulers such as DAPS, BLEST, and ECF were used to demonstrate the efficacy of QAware. It outperformed other schedulers in all network configurations and workloads we tested. %On average, QAware achieves upto $40\%$ increase in throughput for bulk transfers and $30\%$ decrease in fixed-sized file downloads as compared to the default MPTCP scheduler. 
Further, we show that QAware quickly adapts to co-existing applications and sudden variations in network conditions. We have open-sourced QAware's implementation as a modular scheduler for latest stable MPTCP Linux release. 

%For future work, we intend to investigate the effects of MPTCP path schedulers on several other network factors such as congestion at an access point, over-utilization of channel capacity, queueing delay at receiver etc. We believe that several such network aberrations can be overcome by utilizing network-specific aspects, such as congestion, and receiver-specific parameters (such as window size) etc. Explicitly monitoring, predicting and incorporating these parameters with local network variables and TCP-level information is an interesting research question of its own.

%In this paper, we demonstrated the shortcomings of MPTCP scheduling algorithm and the inadequacy of its reliance on SRTT. We proposed the QAware scheduler, which exploits device driver queue occupancy together with sRTT to obtain significantly better performance than the default MPTCP scheduler. We believe that the QAware scheduler highlights the need for a more holistic approach to multipath scheduling than currently being done by MPTCP.% Research is needed for a better understanding how multipath connections should be managed and used, to get better performance and better utilization of the network resources.

%In this paper, we showed the gap in subflow management by Multipath TCP. The current implementation reliance on TCP-level information such as SRTT and congestion window leads to sub-optimal usage of available flow potential. We thus presented QAware, a scheduler for MPTCP which considered device layer queue occupancy for injecting TCP packets in subflows. We implemented QAware scheduler model in NS3 and compared it with the default MPTCP scheduler, minSRTT. We compared the performance of both schedulers in several realistic WiFi and cellular use cases. We observed that QAware can achieve more that 45\% increase in application goodput by incorporating cross-layer information. Finally, we provided a set of cross-flow parameters and network conditions that MPTCP must consider in order to have a more holistic view of it associated network. 


==> discussion.tex <==
\section{Conclusions}


==> motivation.tex <==
\section{Motivation and Problem Statement}

In this section we will motivate the need for minimizing age for status update applications. Using age curve derive the formula for age.
Convince that this is the general formula.

==> protocol.tex <==
\section{Protocol Description}

==> realworld.tex <==
\section{Real World Setup and Results}
We implemented ACP below application layer and used UDP datagrams for communication. We used an Ubuntu 16.04 LTS virtual machine on IIITD server as receiver and an Ubuntu 16.04 LTS machine as a client located outside IIIT-Delhi campus. For communication between these two machines, we established a SSL-VPN connection between the hosts.

==> relatedwork.tex <==
\section{Related Work}


%Starting with~\cite{kaul_minimizing_2011} and~\cite{KaulYatesGruteser-Infocom2012}, there has been growing interest in AoI. While the starting point~\cite{kaul_minimizing_2011} explored  practical issues such as contention window sizes,  the subsequent literature has largely has focused on analytically tractable simple models with updates passing through queues~\cite{NajmInfocom2018Wk}~\cite{ChampatiInfocom2018Wk}~\cite{HuangGLOBECOM2017}~\cite{InoueStationaryDist}, multiple sources sharing a link~\cite{jiang2018timely}~\cite{yates2017status}~\cite{sang2017power}. Papers on scheduling and age optimization REFS have assumed that the system model is known. 
%
%Recently there has been some interest in adaptive approaches that learn how to minimize age across a network etc ... 
%
%I think there is an analogy to the use of HARQ for updates over wireless channels. Both ACP and updates sent using HARQ are trying to adapt to variations in the channel/link. But those HARQ papers tend to  use knowledge of channel statistics to decide when to abandon a transmission. 
%%\cite{van_red}
